A Generalized Kompaneets Formalism for Inelastic Neutrino-Nucleon Scattering in Supernova Simulations

Based on the Kompaneets approximation, we develop a robust methodology to calculate spectral redistribution via inelastic neutrino-nucleon scattering in the context of core-collapse supernova simulations. The resulting equations conserve lepton number to machine precision and scale linearly, not quadratically, with number of energy groups. The formalism also provides an elegant means to derive the rate of energy transfer to matter which, as it must, automatically goes to zero when the neutrino radiation field is in thermal equilibrium. Furthermore, we derive the next-higher-order in {\epsilon}/mc2 correction to the neutrino Kompaneets equation. Unlike other Kompaneets schema, ours also generalizes to the case of anisotropic angular distributions, while retaining the conservative form that is a hallmark of the classical Kompaneets equation. Our formalism enables immediate incorporation into supernova codes that follow the spectral angular moments of the neutrino radiation fields.

==> Generalized Kompaneets/response.tex <==

We very much thank the referee for his/her well-considered comments.  Below, we
address in turn all the issues raised, providing our responses and indicating
the character of the additional text we have added to answer the referee's
questions.  Here, we repeat the referee's points, setting them off with ">"
signs, and follow each with our responses indented.  Hopefully, our responses
and the updates to our manuscript adequately address the issues raised.


> ----------------------------------------------------------------------
> Report of the Referee -- DS12488/Wang
> ----------------------------------------------------------------------
> 
> This work provides a method to calculate the nucleon scattering of
> neutrinos in core-collapse supernovae. The new method appropriately
> treats the effect of momentum and energy transfer that is often
> ignored in numerical simulations despite that it can affect the
> explodability of supernovae. Though this work will benefit the
> community, some issues remain to be fixed before publication.
> 
> Main issues:
> (1)	Difference from Horowitz 2002
> The authors have not cited Horowitz 2002 though it discusses similar
> topics. Horowitz 2002 also discuss the effect of momentum and energy
> transfer on nucleon scattering. First of all, the authors should refer
> to it and discuss the differences of this study from that.

> In Horowitz 2002, he divided the effect of momentum transfer into
> several terms, e.g. phase space and recoil. Are part of them included
> in this work? That is a natural question and the question is important
> since if the answer is YES, then we cannot employ the two schemes
> simultaneously. And if the answer is No, then we can safely include
> both effects. The authors should discuss this topic.

We add the discussions in the conclusion section. Our scheme automatically 
includes the phase space and recoil corrections in Horowitz 2002, because 
our method is based on the dynamic structure function of non-interactive 
nucleons whose low-density limit will give the Horowitz's result. In addition 
to the two corrections above, our result also includs the contribution caused by
the nucleon thermal distribution. 
  
> In addition to that, the authors should mention that s-quark
> correction (Melson+2015) and the correlation by Horowitz 2017 can be
> simultaneously employed or not in their scheme.

Discussions on these two papers are also added in the conclusion part. Correction
in Melson2015 can be included by simply changing the axial-vector coupling constant gA.
Horowitz2017 considers the second virial coefficient, while our scheme only considers
the linear term, so the non-linear terms in Horowitz2017 are not included.
 
> Horowitz 2002:
> https://ui.adsabs.harvard.edu/abs/2002PhRvD..65d3001H/abstract
> Melson+2015:
> https://ui.adsabs.harvard.edu/abs/2015ApJ...808L..42M/abstract
> Horowitz 2017:
> https://ui.adsabs.harvard.edu/abs/2017PhRvC..95b5801H/abstract




> (2)	Final equations to employ
> The authors provide the formula for anisotropic case in section B and
> that for isotropic case with higher correction term in section C.
> There are no unified equations for the anisotropic case with higher
> corrections. It is not convenient for users of this scheme in the
> future. The authors explain the reason in the main text but it would
> be kind to provide expected equations for anisotropic case with higher
> corrections. Maybe (1-lamda) term is added in Eq. (34)-(38).

We have added the anisotropic formulae at the end of the higher order 
correction section. 

> (3)	How to treat boundary of E=0
> In section III, authors demonstrated their method in a numerical way.
> They evaluated second-order differential equations. However, the
> treatment low energy boundary is not written in the text. The authors
> should provide how to treat the boundary of E=0 in the
> demonstration.

We add the boundary condition in the numerical test section. We assume "zero
flux" boundary condition, which means we assume that no particle is scattered outside
the energy range.

> (4)	Qdot in TABLE I and II
> The value of Qdot is not provided by the authors. That value is
> important for users to test their implementation. The authors should
> write the value.

We have added the Qdot values to Table II.

> Minor issues:
> (5)	 Equation numbering
> Equation numbering should be in parenthesis. See the style and
> notation guide. https://cdn.journals.aps.org/files/styleguide-pr.pdf

All numberings are corrected.

> (6)	caption in FIG. 1
> The eq. 3 that the authors write in the caption of FIG.1 is actually
> eq. 2. Please also check other equations.

Figure caption checked.






==> response.tex <==

We very much thank the referee for his/her well-considered comments.  Below, we
address in turn all the issues raised, providing our responses and indicating
the character of the additional text we have added to answer the referee's
questions.  Here, we repeat the referee's points, setting them off with ">"
signs, and follow each with our responses indented.  Hopefully, our responses
and the updates to our manuscript adequately address the issues raised.


> ----------------------------------------------------------------------
> Report of the Referee -- DS12488/Wang
> ----------------------------------------------------------------------
> 
> This work provides a method to calculate the nucleon scattering of
> neutrinos in core-collapse supernovae. The new method appropriately
> treats the effect of momentum and energy transfer that is often
> ignored in numerical simulations despite that it can affect the
> explodability of supernovae. Though this work will benefit the
> community, some issues remain to be fixed before publication.
> 
> Main issues:
> (1)	Difference from Horowitz 2002
> The authors have not cited Horowitz 2002 though it discusses similar
> topics. Horowitz 2002 also discuss the effect of momentum and energy
> transfer on nucleon scattering. First of all, the authors should refer
> to it and discuss the differences of this study from that.

> In Horowitz 2002, he divided the effect of momentum transfer into
> several terms, e.g. phase space and recoil. Are part of them included
> in this work? That is a natural question and the question is important
> since if the answer is YES, then we cannot employ the two schemes
> simultaneously. And if the answer is No, then we can safely include
> both effects. The authors should discuss this topic.

We add the discussions in the conclusion section. Our scheme automatically 
includes the phase space and recoil corrections in Horowitz 2002, because 
our method is based on the dynamic structure function of non-interactive 
nucleons whose low-density limit will give the Horowitz's result. In addition 
to the two corrections above, our result also includs the contribution caused by
the nucleon thermal distribution. 
  
> In addition to that, the authors should mention that s-quark
> correction (Melson+2015) and the correlation by Horowitz 2017 can be
> simultaneously employed or not in their scheme.

Discussions on these two papers are also added in the conclusion part. Correction
in Melson2015 can be included by simply changing the axial-vector coupling constant gA.
Horowitz2017 considers the second virial coefficient, while our scheme only considers
the linear term, so the non-linear terms in Horowitz2017 are not included.
 
> Horowitz 2002:
> https://ui.adsabs.harvard.edu/abs/2002PhRvD..65d3001H/abstract
> Melson+2015:
> https://ui.adsabs.harvard.edu/abs/2015ApJ...808L..42M/abstract
> Horowitz 2017:
> https://ui.adsabs.harvard.edu/abs/2017PhRvC..95b5801H/abstract




> (2)	Final equations to employ
> The authors provide the formula for anisotropic case in section B and
> that for isotropic case with higher correction term in section C.
> There are no unified equations for the anisotropic case with higher
> corrections. It is not convenient for users of this scheme in the
> future. The authors explain the reason in the main text but it would
> be kind to provide expected equations for anisotropic case with higher
> corrections. Maybe (1-lamda) term is added in Eq. (34)-(38).

We have added the anisotropic formulae at the end of the higher order 
correction section. 

> (3)	How to treat boundary of E=0
> In section III, authors demonstrated their method in a numerical way.
> They evaluated second-order differential equations. However, the
> treatment low energy boundary is not written in the text. The authors
> should provide how to treat the boundary of E=0 in the
> demonstration.

We add the boundary condition in the numerical test section. We assume "zero
flux" boundary condition, which means we assume that no particle is scattered outside
the energy range.

> (4)	Qdot in TABLE I and II
> The value of Qdot is not provided by the authors. That value is
> important for users to test their implementation. The authors should
> write the value.

We have added the Qdot values to Table II.

> Minor issues:
> (5)	 Equation numbering
> Equation numbering should be in parenthesis. See the style and
> notation guide. https://cdn.journals.aps.org/files/styleguide-pr.pdf

All numberings are corrected.

> (6)	caption in FIG. 1
> The eq. 3 that the authors write in the caption of FIG.1 is actually
> eq. 2. Please also check other equations.

Figure caption checked.





